Finite Elements with Switch Detection for Numerical Optimal Control of Nonsmooth Dynamical Systems with Set-Valued Heaviside Step Functions

This paper develops high-accuracy methods for numerically solving optimal control problems subject to nonsmooth differential equations with set-valued step functions. A notable subclass of these systems are Filippov systems. The set-valued step functions are here written as the solution map of a linear program. Using the optimality conditions of this problem we rewrite the initial nonsmooth system into a equivalent dynamic complementarity systems (DCS). We extend the Finite Elements with Switch Detection (FESD) method [Nurkanovi\'c et al., 2024], initially developed for Filippov systems transformed via Stewart's reformulation into DCS [Stewart, 1990], to the class of nonsmooth systems with set-valued step functions. The key ideas are to start with a standard Runge-Kutta method for the obtained DCS and to let the integration step sizes to be degrees of freedom. Next, we introduce additional conditions to enable implicit but exact switch detection and to remove possible spurious degrees of freedom if no switches occur. The theoretical properties of the method are studied. Its favorable properties are illustrated on numerical simulation and optimal control examples. All methods introduced in this paper are implemented in the open-source software package NOSNOC.

==> sections/step_representation.tex <==
\section{Nonsmooth systems with set-valued step functions}
In this section, we show how to rewrite a step function as a solution map of a linear program.
In section \ref{sec:no}, we introduce the general differential inclusions studied in this paper.
Section \ref{sec:filippov_sys} specializes on Filippov systems and derives an equivalent DCS.
\subsection{Set-valued step functions}
The set-valued step function $\gamma : \R \to \mathcal{P}(\R)$ is defined as:
\begin{align}\label{eq:step_function}
	\gamma(y) &= \begin{cases}
		\{1\},\ &y>0, \\
		[0,1],\ &y=0, \\
		\{0\},\ &y<0.
	\end{cases}
\end{align}
The vector-valued version of the step function, denoted by $\Gamma: \R^{n_y} \to \mathcal{P}(\R^{n_y})$ is the concatenation of scalar step functions, i.e., for $y \in \R^{n_y}$ we have
$\Gamma(y)= (\gamma(y_1),\dots,\gamma(y_{n_y})) \in \R^{n_y}$.
Let us denote by $\alpha \in \R^{n_c}$ a selection $\alpha \in \Gamma(y)$.

Let $c(x)$ be a continuous function of $x$, where $x(t)$ is some continuous function of time.
In the literature well-known way to express the function $\Gamma(c(x))$~\cite{Acary2014,Baumrucker2009} is the use of
the solution map of the parametric linear program:
\begin{subequations}\label{eq:step_parametric_lp}
	\begin{align}
		\Gamma(c(x))  = \arg \min_{\alpha\in \R^{n_c}} \ &-c(x)\alpha \\
		\quad \mathrm{s.t.} \quad & 0 \leq \alpha_i \leq 1, \ i=1,\ldots,n_c \label{eq:step_parametric_lp_ineq}.
	\end{align}
\end{subequations}
%This variant is in NOSNOC labeled as \texttt{StepLinear}.
Note that all components of $\alpha$ are decoupled in this LP, i.e., every $\alpha_i$ can be obtained by solving a one-dimensional LP with the objective $-c_i(x)\alpha_i$ and the feasible set $0\leq \alpha_i \leq 1$.
Let $\lambdan,\lambdap \in \R^{n_c}$ be the Lagrange multipliers for the lower and upper bound on $\alpha$ in \eqref{eq:step_parametric_lp_ineq}, respectively.
The KKT conditions of \eqref{eq:step_parametric_lp} read as
\begin{subequations}\label{eq:step_parametric_lp_kkt}
	\begin{align}
		&c(x) = \lambdap - \lambdan, \label{eq:step_parametric_lp_kkt_lagrangian}\\
		&0 \leq  \lambdan \perp \alpha \geq 0,\\
		&0 \leq  \lambdap \perp e-\alpha \geq 0,
	\end{align}
\end{subequations}
Let us look at a single component $\alpha_j$ and the associated functions $c_j(x)$.
From the LP \eqref{eq:step_parametric_lp} and its KKT conditions, one can see that for $c_j(x) > 0$, we have $\alpha_j=1$.
Since the upper bound is active, we have that $\lambda_{\mathrm{n},j} = 0$ and from \eqref{eq:step_parametric_lp_kkt_lagrangian} that $\lambda_{\mathrm{p},j} = c_j(x) > 0$.
Likewise, for $c_j(x) < 0$, we obtain $\alpha_j=0$, $\lambda_{\mathrm{p},j} = 0$ and $\lambda_{\mathrm{n},j} = -c_j(x) > 0$.
On the other hand, $c_j(x) = 0$ implies that $\alpha_j \in [0,1]$ and $\lambda_{\mathrm{p},j} = \lambda_{\mathrm{n},j} = 0$.
From this discussions, in can be seen that $c(x)$, $\lambdan$ and $\lambdap$ are related by following expressions:
\begin{subequations}\label{eq:step_continuity_lambda}
	\begin{align}
		\lambdap &= \max(c(x),0),\\
		\lambdan &= -\min(c(x),0).
	\end{align}
\end{subequations}
That is, $\lambdap$ collects the positive parts of $c(x)$ and $\lambdan$ the absolute value of the negative parts of $c(x)$.
From this relation, we have immediately the following fact.
\begin{lemma}
	Let $c(x(t))$ be a continuous function of time, then the functions $\lambdap(t)$ and $\lambdan(t)$ are continuous in time.
\end{lemma}

%
%Alternatively, one can replace the two linear constraints in \eqref{eq:step_parametric_lp_ineq} per component with a single equivalent conic constraint and a parametric convex program:
%\begin{subequations}\label{eq:step_parametric_cp}
%	\begin{align}
%		\Gamma(c(x))  = \arg \min_{\alpha\in \R^{n_c}} \ &-c(x)\alpha \\
%		\quad \mathrm{s.t.} \quad &\Big(\alpha_i-\frac{1}{2}\Big)^2 \leq \Big(\frac{1}{2}\Big)^2,\ i = 1,\ldots,n_c. \label{eq:step_parametric_cp_ineq}
%	\end{align}
%\end{subequations}
%To the best of our knowledge, this formulation is barely used in the literature, but we show below that it has some computational advantages.
%This variant is in NOSNOC labeled as \texttt{StepConic}.
%Let $\lambdaa \in \R^{n_c}$ be the Lagrange multiplier of \eqref{eq:step_parametric_cp_ineq}.
%The KKT conditions of \eqref{eq:step_parametric_cp} reads as:
%\begin{subequations}\label{eq:step_parametric_cp_kkt}
%	\begin{align}
%		&c_i(x) = \lambdaa_i (2\alpha_i-1),\ i = 1,\ldots,n_c,\\
%		&0 \leq  \lambdaa_i \perp \frac{1}{4}-\Big(\alpha_i-\frac{1}{2}\Big)^2 \geq 0,\ i = 1,\ldots,n_c.
%	\end{align}
%\end{subequations}
%Since $\alpha_i \in [0,1]$, it is not difficult to see that:
%\begin{align*}
%	&|c_i(x)| = \lambdaa_i,\ i = 1,\ldots,n_c.
%\end{align*}
%From this equation, the following facts follow immediately.
%\begin{lemma}
%	Let $c(x(t))$ be a continuous function of time, then the function $\lambdaa(t)$ is continuous in time.
%\end{lemma}
%Note that the components of \eqref{eq:step_parametric_lp_ineq} represent the $\ell_1$ ball centered at $\frac{1}{2}$ with the radius $\frac{1}{2}$, whereas in \eqref{eq:step_parametric_cp_ineq} we have the same ball but in the two-norm.
%The advantage of the conic formulation over the linear one is that it has only one complementarity condition in its KKT condition.
%However, one of the functions entering the complementarity conditions in the conic case is quadratic.
%For brevity, we do all derivations for the parametric LP case.
%However, all extensions to the conic case are straightforward.
%\subsection{Differential inclusions with set-valued step functions}\label{sec:step_representation}
%\todo{give an outline of this section}
\subsection{Aizerman–Pyatnitskii differential inclusions}
The set-valued step functions allow the formulation of DIs more general than Filippov systems:
\begin{align}\label{eq:di_ap}
	\dot{x} \in F(x,u,\Gamma(c(x))),
\end{align}
where $c:\R^{n_x} \to \R^{n_c}$ are \textit{switching functions}.
The components of the function $\Gamma(c(x))$ can be related in a complicated nonlinear way.
These systems are sometimes called Aizerman–Pyatnitskii differential inclusions, cf. \cite{Acary2014} and \cite[page 55, Definition c]{Filippov1988}.
Time-stepping methods for such systems were developed in \cite{Acary2014}.
Such systems do not have a rich theory as Filippov DIs and there are fewer results on the existence of solutions and convergence of numerical methods available \cite{Acary2014}.
From the derivations below it will become apparent that Filippov systems are a special case of \eqref{eq:di_ap}.
Using one of the KKT systems \eqref{eq:step_parametric_lp_kkt} and \eqref{eq:step_parametric_cp_kkt}, the DI \eqref{eq:di_ap} can readily be transformed into a dynamic complementarity system.
The numerical methods in this paper mainly exploit the continuity properties of the Lagrange multipliers in these KKT systems and thus are directly applicable to \eqref{eq:di_ap}.
However, we restrict our theoretical studies to the case of Filippov systems, as they have a richer theory that we can build upon.

\subsection{Filippov set expressed via step functions}\label{sec:step_dcs}
We regard piecewise smooth systems in the form of
\begin{align} \label{eq:pss}
	\dot{x}(t) = f_i(x(t),u(t)),\ &\mathrm{if} \  x(t) \in R_i \subset \R^{n_x}, \\
	&i \in \mathcal{J} \coloneqq \{ 1,\dots,\Nsys  \},
\end{align}
where $R_i$ are disjoint, connected, and open sets.
They are assumed to be nonempty and to have piecewise-smooth boundaries $\partial R_i$.
We assume that $\overline{\bigcup\limits_{i\in \mathcal{J}} R_i} = \R^{n_x}$ and that $\R^{n_x} \setminus \bigcup\limits_{i\in\mathcal{J}} R_i$ is a set of measure zero.
The functions $f_i(\cdot)$ are assumed to be Lipschitz and at least twice continuously differentiable functions on an open neighborhood of $\overline{R}_i$.
Furthermore, $\Nsys$ is a positive integer, and $u(t)$ is a sufficiently regular externally chosen control function.

The ODE \eqref{eq:pss} is not defined on the region boundaries $\partial R_i$.
Classical notions of solution are suitable for \eqref{eq:pss}, especially if the trajectories have so-called \textit{sliding modes}, i.e., when $x(t)$ must evolve on $\partial R_i$ \cite{Cortes2008,Filippov1988}.
Therefore, we regard Filippov's convexification of \eqref{eq:pss}.
Moreover, the special structure of the PSS allows the definition of a finite number of convex multipliers $\theta_i$, such that Filippov's DI
is defined as \cite{Filippov1988,Stewart1990a}:
\begin{align}\label{eq:filippov_di_with_multiplers}
	\dot{x}  \in F_{\mathrm{F}}(x,u) = \Big\{ &\sum_{i\in \mathcal{J}}
	f_i(x,u) \, \theta_i  \mid \sum_{i\in \mathcal{J}}\theta_i = 1,  \\
	\ &\theta_i \geq 0,
	\ \theta_i = 0 \  \mathrm{if} \;  x \notin \overline{R}_i,
	\forall  i  \in \mathcal{J} \Big\}. \nonumber
\end{align}
The basic question to be answered is: How can we find an (implicit) function that calculates the Filippov multipliers $\theta$ for a given $x$?

To derive such functions, we will make use of the set-valued step functions and the definition of the regions $R_i$, which are expressed via the switching functions $c_j(x)$.
We assume the functions $c_j(\cdot)$ to be Lipschitz continuous, sufficiently differentiable and that $\nabla c(x) \in \R^{n_x\times {n_c}}$ has rank ${n_c}$.
With $n_c$ scalar functions we define up to $n_f =2^{n_c}$ regions:
\begin{align*}
	R_1 &= \{x \in \R^{n_x}  \mid c_1(x) >0,c_2(x) >0, \ldots, c_{n_c}(x) >0 \},\\
	R_2 &= \{x \in \R^{n_x}  \mid c_1(x) >0,c_2(x) >0, \ldots, c_{n_c}(x) <0 \},\\
	\vdots\\
	R_{n_f} &= \{x \in \R^{n_x}  \mid c_1(x) <0,c_2(x) <0, \ldots, c_{n_c}(x) <0 \}.
\end{align*}
%Each region $R_i$ is equipped with a vector field $f_i(x),\; i \in \{1,\ldots,n_f\}$.
%Same as in the Stewart reformulation
These definitions are compactly expressed via a dense sign matrix $S \in \R^{\Nsys \times n_c}$:
\begin{align}\label{eq:sign_matrix}
	S = \begin{bmatrix}
		1 & 1 & \dots &1 & 1\\
		\vdots &  \vdots & \cdots &  \vdots &  \vdots\\
		-1 & -1 & \dots & 1& 1\\
		-1 & -1 & \dots & 1& -1\\
	\end{bmatrix}.
\end{align}
The matrix $S$ has no repeating rows and no zero entries.
We define the index set of all switching functions $\mathcal{C} = \{1,\ldots,n_c\}$.
The sets $R_i$ can be compactly represented using the rows of the matrix $S$:
\begin{align}\label{eq:standard_sets_step_dense}
	R_i &= \{ x\in \R^{n_x} \mid S_{i,j} c(x)>0, j \in \mathcal{C} \}.
\end{align}
Note that the boundaries of the regions $\partial R_i $ are subsets of the zero-level sets of appropriate functions $c_j(x)$.
Moreover, if the definition of some set $R_i$ does not depend on some functions $c_j(x)$, then we can express the definition of ${R}_i$ via a sparse matrix.
We denote this matrix by $\hat{S} \in \R^{\Nsys \times n_c}$.
An example reads as
\begin{align}\label{eq:sparse_sign_matrix}
	\hat{S} = \begin{bmatrix}
		1 & 0 & \dots &0 & 0\\
		\vdots &  \vdots & \cdots &  \vdots &  \vdots\\
		-1 & -1 & \dots & 1& 0\\
		-1 & -1 & \dots & 1& -1\\
	\end{bmatrix}.
\end{align}
It is not allowed that this matrix to have a row with all zeros.
The sparsity in the matrix $\hat{S}$ arises from the geometry of the regions $R_i$.
For every region $R_i$, we define an index set containing the indices of all switching functions relevant for its definition, i.e.,
\begin{align*}
 \mathcal{C}_i = \{ j \in  \mathcal{C} \mid \hat{S}_{i,j}\neq 0\}, \textrm{ for all } i \in \mathcal{J}.
\end{align*}
Now, the matrix $\hat{S}$ enables us to compactly express the definitions of the regions $R_i$ as:
 \begin{align}\label{eq:standard_sets_step}
	{R}_i &= \{ x\in \R^{n_x} \mid \hat{S}_{i,j} c_j(x)>0,\; j \in \mathcal{C}_i\}.
\end{align}

%The closure of the regions $R_i$ can be expressed via $\hat{S}$ in a similar way to \eqref{eq:standard_sets_step_dense}:
% \begin{align*}
%% 	\label{eq:standard_sets_closure}
%	\overline{R}_i &=\{ x\in \R^{n_x} \mid \mathrm{diag} (\hat{S}_{i,\bullet}) c(x)\geq0\}.
%\end{align*}
%In the sequel, we work with the definition in Eq. \eqref{eq:standard_sets_step}.

This new representation via the matrix $\hat{S}$ might seem to complicate things.
The effort we invested here for additional definitions via a sparse matrix $\hat{S}$ will pay off in the step representation, as we can reduce the number of algebraic variables and improve the computational efficiency.
This will become apparent in some of the examples given below.
Let us first illustrate the development so far with an example.


\begin{example}[Compact representation of regions]\label{ex:sparse_sets}
We regard three regions defined via two scalar switching functions $c_1(x)$ and $c_2(x)$:
$R_1 = \{ x\in \R^{n_x} \mid c_1(x) > 0\},\;
R_2 = \{ x\in \R^{n_x} \mid  c_1(x) < 0, c_2(x)>0\}$ and
$R_3 = \{ x \in \R^{n_x}  \mid c_1(x) < 0, c_2(x)<0\}$.
It is not difficult to see, that by using Eq. \eqref{eq:standard_sets_step} these sets can be compactly defined by
\begin{align*}
  \hat{S} = \begin{bmatrix}
  	1& 0\\
  	-1& 1\\
  	-1&-1
  \end{bmatrix}.
\end{align*}
However, sometimes a matrix with no zero entries is needed.
For example, this is required in Stewart's representation of Filippov systems outlined in Section \ref{sec:stewarts_representation}.
To obtain a matrix with nonzero entries we must introduce some redundancy and extend matrix $\hat{S}$ as follows.
By noting that
$R_1 = \{ x\in \R^{n_x} \mid c_1(x) > 0\} =  \{ x \in \R^{n_x} \mid c_1(x) > 0, c_2(x)<0\} \cup \{ x\in \R^{n_x} \mid c_1(x) > 0, c_2(x)\geq0\}$,
we can construct a dense matrix:
\begin{align*}
	{S} = \begin{bmatrix}
		1& 1\\
		1& -1\\
		-1& 1\\
		-1&-1
	\end{bmatrix},
\end{align*}
and define
$R_i' = \{ x\in \R^{n_x} \mid \mathrm{diag} (S_{i,\bullet}) c(x)>0\}, i \in \{1,\ldots,4\}$.
It can be seen
$R_1 = R_1' \cup R_2' \cup R_1^{\mathrm{res}}$,
$R_2 = R_3' $ and
$R_3 = R_4'$,
where $R_1^{\mathrm{res}} = \{x\mid c_1(x)>0,c_2(x)=0\}$, i.e., the boundary between $R_1'$ and $R_2'$.
It is important to note that the set of measure zero $R_1^{\mathrm{res}}$ was added to $R_1$ as it was excluded by the definition via strict inequalities.
However, in a Filippov setting, we anyway have the same vector field $f_1(x)$ in both $R_1'$ and $R_2'$.
Thus, it follows directly from the definition in Eq. \eqref{eq:filippov_set} that for all $x \in R_1^{\mathrm{res}}$ is $F_{\mathrm{F}}(x) = \{f_1(x)\}$, which is consistent with a more compact representation.
\end{example}





For ease of exposition, we illustrate the step representation on a simple example and give in the sequel the general expression.
\begin{example}[Step representation]
Regard the sets $R_i$, $i\in \{1,\ldots,3\}$ as in Example \ref{ex:sparse_sets} and the associated vector fields $f_i(x),i\in \{1,\ldots,3\}$.
Let $\alpha \in \Gamma(c(x)) \in \R^2$.
A selection of the Filippov set \eqref{eq:filippov_di_with_multiplers} and the associated ODE reads as:
\begin{align*}
	\dot{x} = \alpha_1 f_1(x)  \!+\! (1-\alpha_1)\alpha_2 f_2(x) \!+\! (1-\alpha_1)(1-\alpha_2) f_3(x).
\end{align*}
By inspection we determine that $\theta_1 = \alpha_1$, $\theta_2 = (1-\alpha_1)\alpha_2$ and $\theta_3 = (1-\alpha_1)(1-\alpha_2)$.
Since $\alpha_1, \alpha_2 \in [0,1]$ it is clear that $\theta_i \in [0,1], i\in \{1,\ldots,3\}$.
Similarly, direct calculation shows that $\theta_1 + \theta_2 + \theta_3 = 1$.
We conclude, that we have indeed represented the Filippov set with the expression above.
Observe that the entries of $\hat{S}_{i,j}$ determine how $\alpha_j$ enters the expression for $\theta_i$.
For $\hat{S}_{i,j} =1$ we have $\alpha_j$, for $\hat{S}_{i,j} =-1$ we have $(1-\alpha_j)$ and for $\hat{S}_{i,j} =0$, $\alpha_j$ does not appear in the expression for $\theta_i$.
This leads to multi-affine terms consisting of products of $\alpha_j$ and $(1-\alpha_j)$.
Next, let us verify on a few examples that $\theta_i$ also takes the correct values.
For $x \in R_1$ we have that $\alpha_1 = 1$, whereas $\alpha_2$ can take any value in $[0,1]$. In this case
$\theta_1 =1$ and $\theta_2 = \theta_3 = 0$.
Now let $\I(x) = \{1,2\}$, that is we have a sliding mode between $R_1$ and $R_2$, i.e.,  $c_1(x)=0$ and $c_2(x) >0$.
Thus we obtain, $\theta_1 \in [0,1]$, $\theta_2 \in [0,1]$ and $\theta_3 = 0$.
The values of $\theta_1$ and $\theta_2$ are determined from the condition $\frac{\dd}{\dd t } c_1(x) = 0$.
\end{example}

We generalize the patterns observed in the last example and define the set
%\begin{align}\label{eq:step_set}
%		F_{\mathrm{S}}(x) &\coloneqq \Big\{ \sum_{i=1}^{\Nsys} \prod_{j=1}^{n_c} 2^{n_{c}-n_{R_i}} 	\Big( \frac{1-\hat{S}_{i,j}}{2}+\hat{S}_{i,j}\alpha_i \Big) f_i(x) \mid \alpha \in \Gamma(c(x)) \Big\}.
%\end{align}
\begin{align}\label{eq:step_set}
	F_{\mathrm{S}}(x) &\coloneqq\\
	\nonumber &\Big\{ \sum_{i=1}^{\Nsys} \prod_{j \in \mathcal{C}_i} 	\Big( \frac{1-\hat{S}_{i,j}}{2}+\hat{S}_{i,j}\alpha_i \Big) f_i(x) \mid \alpha \in \Gamma(c(x)) \Big\}.
\end{align}
Note that we have
%\begin{align*}
%	\frac{1-\hat{S}_{i,j}}{2}+\hat{S}_{i,j}\alpha_i	&= \begin{cases}
%		\alpha_i,\ & \hat{S}_{i,j} = 1, \\
%		\frac{1}{2},\ &\hat{S}_{i,j} = 0, \\
%		1-\alpha_i,\ &\hat{S}_{i,j} = -1.
%	\end{cases}
%\end{align*}
\begin{align*}
	\frac{1-\hat{S}_{i,j}}{2}+\hat{S}_{i,j}\alpha_i	&= \begin{cases}
		\alpha_i,\ & \textrm{ if } \hat{S}_{i,j} = 1, \\
		1-\alpha_i,\ & \textrm{ if }  \hat{S}_{i,j} = -1.
	\end{cases}
\end{align*}
%If $\hat{S}_{i,j} = 0$, then the definition of the region $R_i$ does not depend on $c_j(x)$, but it depends only on $n_{R_i} = \sum | \hat{S}_{i,\bullet}| \leq n_c$ components of $c(x)$.
%Thus, the term $2^{{n_c}-n_{R_i}}$ compensates the effect of the accumulated products of $\frac{1}{2}$ due to the zero entries of $\hat{S}_{i,\bullet}$.
Similar definitions of $F_{\mathrm{S}}(x)$ in Eq. \eqref{eq:step_set} can be found in \cite[Section 4.2]{Dieci2011} and \cite[Section 2.1]{Guglielmi2022}.
However, they are restricted to fully dense matrices $S$ and do not derive the relation to a DCS.
These works focus on explicitly computing the selections $\alpha$ for a given fixed active set \cite{Dieci2011} or to use a smooth single-valued approximation of $\Gamma(x)$ for simulation purposes \cite{Guglielmi2022}.
Next we show that $F_{\mathrm{S}}(x)$ is indeed the same set as $F_{\mathrm{F}}(x)$, i.e., the set in the r.h.s. of \eqref{eq:filippov_di_with_multiplers}.

%Let \begin{align}\label{eq:theta_via_step}
	%	\theta_i &= 2^{n_{c}-n_{R_i}}  \prod_{j=1}^{n_c}  \frac{1-\hat{S}_{i,j}}{2}+\hat{S}_{i,j}\alpha_j,
	%	%	\theta_i = 2^{n_{c}-n_{R_i}}  \det(\mathrm{diag}((\frac{1}{2}(e-S_{i,\bullet})+\mathrm{diag}(S_{i,\bullet})\alpha))
	%\end{align}
\begin{lemma}[Lemma 1.5 in \cite{Dieci2011}]\label{lem:dieci}
Let $a_1,a_2,\ldots a_m \in \R$. Consider the $2^m$ non-repeated products of the form
$p_i = (1\pm a_1)(1\pm a_2)\cdots(1\pm a_m)$, then it holds that $\sum_{i}^{2^m} p_i = 2^m$.
\end{lemma}
\begin{proposition}
Let \begin{align}\label{eq:theta_via_step}
	\theta_i &= \prod_{j\in \C_i}  \frac{1-\hat{S}_{i,j}}{2}+\hat{S}_{i,j}\alpha_j,
\end{align}
for all $i\in \mathcal{J} = \{1,\ldots,\Nsys\}$, then it holds that $F_{\mathrm{F}}(x)$ = 	$F_{\mathrm{S}}(x)$.
\end{proposition}
\textit{Proof.}
We only need to show that $\theta_i \geq 0$ for all $i \in \J$ and $\sum_{i\in \J} \theta_i  =1$.
It is easy to see that $\theta_i\in [0,1]$ as it consists of a product of terms that takes value in $[0,1]$.


Next we show that $\sum_{i\in \mathcal{J}} \theta_i  =1$.
We introduce the change of variables:
\begin{align*}
\frac{1+b_j}{2} &= \alpha_j,\; \frac{1-b_j}{2}= 1-\alpha_j.
\end{align*}
Then all $\theta_i$ are of the form
\begin{align*}
\theta_i = 2^{-|\C_i|} \prod_{j \in \C_i}  (1\pm b_j).
\end{align*}
If the matrix $\hat{S}$ is dense we have that $\C_i = \C$ for all $i \in\mathcal{J}$ and $\Nsys = 2^{n_c}$.
By applying Lemma \ref{lem:dieci} we conclude that $\sum_{i\in \mathcal{J}}\theta_i=1$ and the proof is complete.


On the other hand, if the matrix $\hat{S}$ has zero entries we have that $\Nsys < 2^{n_c}$.
We extend sequence $\{\theta_i\}_{i=1}^{n_f}$ to  $\{\tilde{\theta}_l\}_{l=1}^{2^{n_c}}$, where the terms $\tilde{\theta}_l$ are defined as follows.
If $\C_i = \C$, then $\tilde{\theta}_i = \theta_i$.
Now let $\C_i \subset \C$ and $\C \setminus \C_i = \{ k\}$, i.e., only one $\hat{S}_{i,k}$ in $\hat{S}_{i,\bullet}$ is zero.
We can use the simple identity $\theta_i = \theta_i \frac{(1+b_k)}{2}+\theta_i \frac{(1-b_k)}{2}$, and let two additional $\tilde{\theta}_{l}$ be the two terms in the extended sum above.
Applying this procedure inductively we obtain for all $i$ where $\C_i \subset \C$ terms $\tilde{\theta}_l$ of the form $\frac{(1\pm b_1)}{2}\cdots\frac{(1\pm b_{n_c})}{2}$.
Now we can apply Lemma \ref{lem:dieci} and conclude that $\sum_{i=1}^{n_f} \theta_i = \sum_{l=1}^{2^{n_c}} \tilde{\theta}_l = 1$.
\qed



To pass from the definition in Eq. \eqref{eq:step_set} to a dynamic complementarity system, we the KKT conditions of \eqref{eq:step_parametric_lp} to obtain an algebraic expression for $\Gamma(c(x))$.
%$\Gamma(\cdot)$ as the solution map of the parametric linear program:
%\begin{subequations}\label{eq:step_parametric_lp}
%\begin{align}
%	\Gamma(c(x))  = \arg \min_{\alpha\in \R^{n_c}} \ &-c(x)\alpha \\
%	\quad \mathrm{s.t.} \quad &0 \leq \alpha \leq e \label{eq:step_parametric_lp_ineq}.
%\end{align}
%\end{subequations}
%Note that all the components of $\alpha$ are decoupled in this LP, i.e., every $\alpha_i$ can be obtained by solving a one-dimensional LP with the objective $-c_i(x)\alpha_i$ and the feasible set $0\leq \alpha_i \leq 1$.
%Let $\lambdan,\lambdap \in \R^{n_c}$ be the Lagrange multipliers for the lower and upper bound on $\alpha$ in \eqref{eq:step_parametric_lp_ineq}, respectively.
Using the KKT condition of the LP representation \eqref{eq:step_parametric_lp_kkt}, the definition of the Filippov set in \eqref{eq:step_set} and the expression for $\theta_i$ in \eqref{eq:theta_via_step}, we obtain the following DCS:
\begin{subequations}\label{eq:step_dcs}
	\begin{align}
		&\dot{x} = F(x,u)\; \theta, \\
		%    	&\theta_i = 2^{n_{c}-n_{R_i}}  \prod_{j=1}^{n_c}  \frac{1-\hat{S}_{i,j}}{2}+\hat{S}_{i,j}\alpha_j,\; \textrm{for all } i\in\mathcal{J},\\
		&\theta_i = \prod_{j\in \C_i}  \frac{1-\hat{S}_{i,j}}{2}+\hat{S}_{i,j}\alpha_j,\; \textrm{for all } i\in \J,\\
		&c(x) = \lambdap - \lambdan,\label{eq:step_dcs_lp_lagrangian}\\
		&0 \leq  \lambdan \perp \alpha \geq 0,\\
		&0 \leq  \lambdap \perp e-\alpha \geq 0,
	\end{align}
\end{subequations}
where $F(x) = [f_1(x,u),\dots, f_{\Nsys}(x,u)] \in \R^{n_x \times \Nsys}$, $\theta =(\theta_1,\dots,\theta_{\Nsys}) \in \R^{\Nsys}$ and $\lambdap,\lambdan,\alpha \in \R^{n_c}$.

We group all algebraic equations into a single function and use a C-function $\Psi(\cdot,\cdot)$ for the complementarity condition to obtain a more compact expression:
\begin{align}\label{eq:dcs_step_lp}
	G(x,\theta,\alpha,\lambdap,\lambdan) \coloneqq
	\begin{bmatrix}
		\theta_1 - \prod_{j \in C_1}  \frac{1-\hat{S}_{1,j}}{2}+\hat{S}_{1,j}\alpha_j\\
		\vdots\\
		\theta_{n_f} - \prod_{j \in C_{n_f}}  \frac{1-\hat{S}_{n_f,j}}{2}+\hat{S}_{n_f,j}\alpha_j\\
		c(x) - \lambdap + \lambdan\\
		\Psi( \lambdan,\alpha)\\
		\Psi( \lambdap,e-\alpha)
	\end{bmatrix}.
\end{align}
Finally, we obtain a compact representation of \eqref{eq:step_dcs} in the form of a nonsmooth DAE:
\begin{subequations}\label{eq:dcs_step_2}
	\begin{align}
		\dot{x} & = F(x,u)\theta,\\
		0&= 	G(x,\theta,\alpha,\lambdap,\lambdan).
	\end{align}
\end{subequations}


Regarding the sensitivities w.r.t. parameters for the DCS obtained via the step reformulation, we note that
one can make almost an identical analysis as in Section \ref{sec:sensitivites_pss} if the function $\psi_{i,j}(\cdot)$ is replaced by an appropriate switching function $c_k(\cdot)$.
We remind the reader that all derivations above could be carried out with the conic representation in Eqs. \eqref{eq:step_parametric_cp} and \eqref{eq:step_parametric_cp_kkt}.

\subsection{Stewart's representation}\label{sec:stewarts_representation}
In Stewart's representations the regions $R_i$ are defined via so-called indicators functions $g_i(x)$ for all $i \in \mathcal{I}$. The definition reads as
\begin{align}\label{eq:stewart_sets}
	R_i = \{ x \in \R^{n_x} \mid g_i(x) < \min_{j\in \mathcal{I}\setminus\{i\}} g_j(x)\}.
\end{align}
This representation of the regions might not be the most intuitive one.
However, it was shown in \cite{Nurkanovic2022} that the function $g(x)$ can be obtained as:
\begin{align}\label{eq:stewart_indicators}
	g(x) = -S c(x).
\end{align}
Stewart's reformulation of Filippov systems into DCS requires the matrix $S$ to have nonzero entries.
The multipliers $\theta$ is expressed as the solution of an LP parameterized by $x$:
\begin{subequations}\label{eq:stewart_lp}
	\begin{align}
		\quad \theta(x)  \in\arg\min_{\tilde{\theta} \in \R^{\Nsys}} \quad & g(x)^\top \, \tilde{\theta} \\
		\textrm{s.t.} \quad & e^\top \tilde{\theta} = 1
		\\
		&\tilde{\theta}\geq 0.
	\end{align}
\end{subequations}
Using its KKT condition, one can obtain a DCS similar to \eqref{eq:dcs_step_2}.
The FESD method was initially developed for this formulation in \cite{Nurkanovic2022}.

It can be shown by direct verification (e.g., in Example \ref{ex:sparse_sets}), that equation \eqref{eq:stewart_indicators} does not provide the correct $g(x)$ if we use a sparse matrix $\hat{S}$ instead of $S$.
Thus, we cannot represent Filippov sets via Stewart's approach if we use $\hat{S}$.
Instead, we must construct an appropriate larger and dense matrix $S$ to encode the regions, cf. Example \ref{ex:sparse_sets}.
This results in more algebraic variables, as we need more indicator functions $g_i(\cdot)$.
In examples the dense representation is the most compact one, i.e., $\hat{S} = S$ and in this case, Stewart's representation introduces no redundancy.
%\section{Properties of the dynamics complementarity systems}


\section{Properties of the DCS}\label{sec:dcs_properties}
\subsection{Active-set changes and continuity of $\lambdap$ and $\lambdan$}
\label{sec:step_dcs_active_set_changes}
Active-set changes are paired with discontinuities in some of the algebraic variables.
We have seen above that $\lambdap$ and $\lambdan$ are continuous functions of time.
We can exploit this property in the development of numerical simulation methods in the next chapter.

At an active-set change, we have a zero-crossing of the switching functions $c_j(x)$.
It follows from \eqref{eq:step_continuity_lambda} that also $\lambda_{\mathrm{p},j}(t)$ and $\lambda_{\mathrm{n},j}(t)$ must be zero at an active-set change.
We use the now DCS formulation via step functions in Eq. \eqref{eq:step_dcs} to illustrate
the different switching cases that arise in Filippov systems.
\begin{example}\label{ex:switching_cases}
	There are four possible switching cases which we illustrate with the following examples:
	\begin{enumerate}[(a)]
		\item crossing a surface of discontinuity, $\dot{x}(t) \in 2-\mathrm{sign}(x(t))$,
		\item sliding mode, $\dot{x}(t) \in -\mathrm{sign}(x(t))+0.2\sin(5t)$,
		\item leaving sliding mode $\dot{x}(t) \in -\mathrm{sign}(x(t))+t$,
		\item spontaneous switch, $\dot{x}(t) \in \mathrm{sign}(x(t))$.
	\end{enumerate}
	In case (a), for $x(0) < 0$ the trajectory reaches $x = 0$ and crosses it.
	In example (b), for any finite $x(0)$, the trajectory reaches $x=0$ and stays there.
	On the other hand, in example (c), for $x(0) =0$, the DI has a unique solution and leaves $x=0$ at $t=1$.
	In the last example, for $x(0) =0$ the DI has infinitely many solutions, and $x(t)$ can spontaneously leave $x = 0$ at any $t\geq0$.
	The trajectories are illustrated in Figure \ref{fig:switcing_cases_step}.
	In all cease the Lagrange multipliers $\lambdap$ and $\lambdan$ are zero at a switch but have nonzero left or right time derivatives.
\end{example}
\begin{figure}[t]
		\centering
		{\includegraphics[scale=0.45]{image/step_crossing.pdf}}
		{\includegraphics[scale=0.45]{image/step_sliding_mode.pdf}}
		{\includegraphics[scale=0.45]{image/step_leaving.pdf}}
		{\includegraphics[scale=0.45]{image/step_spontaneous.pdf}}
		\caption{
			Illustration of example solution trajectories for different switching cases.
			The rows from top to bottom show $x(t)$, $\alpha(t)$, $\lambdap(t)$ and  $\lambdan(t)$ for the cases (a)-(d) in Example~\ref{ex:switching_cases}, respectively.
		}
		\label{fig:switcing_cases_step}
	\end{figure}
\subsection{Fixed active set in the step formulation}\label{sec:step_dcs_active_set_fixed}
Recall that for a given solution $x(\cdot)$ the fixed active set between two switches is denoted by $\I_n\coloneqq \I(x(t)), \ t\in (t_{\mathrm{s},n},t_{\mathrm{s},n+1})\eqqcolon \mathcal{T}_n$.
We study the properties of the DCS \eqref{eq:step_dcs} for a fixed active set $\mathcal{I}_n$, which we, for brevity, denote by $\I$.
Without loss of generality, the corresponding time interval is $\mathcal{T} = (0,T)$.
For a fixed active set, the DCS \eqref{eq:step_dcs} reduces either to an ODE or to a DAE.


We start with the simpler ODE case.
Let $c_j(x) \neq 0$ for all $j \in \C$, then $x(t)$ is in the interior of some region $R_i$.
It can be seen from the LP \eqref{eq:step_parametric_lp} that $\alpha_j \in \{0,1\}$ for all $j \in \C$.
This implies that $\theta_i=1$ and $\theta_k = 0, k \neq i$.
Therefore, $\I  = \{i\}$ and in this case, the Filippov DI reduces to $\dot{x} \in F_{\mathrm{F}}(x) = \{f_i(x)\}$, i.e., we have locally an ODE which is consistent with the developments so far.

Next, we regard the case when $\I$ is not a singleton.
This means that we are at the boundary of two or more regions.
Consequently, we have at least one $c_j(x)=0$.
Let us associate with $\I$ the index set $\K  = \{ j \in \C \mid  c_j(x) = 0\}$, i.e., the set of indices of all switching functions that are zero for a given active set $\I$.
Following the discussion from the previous section, for all nonzero $c_j(x)$, i.e., $j \in \C \setminus \K$, we can compute $\alpha_j \in \{0,1\}$ via the LP \eqref{eq:step_parametric_lp} and $\lambda_{\mathrm{p},j}, \lambda_{\mathrm{n},j}$ via Eq. \eqref{eq:step_continuity_lambda}.
Next, we have that $\lambda_{\mathrm{p},j} = \lambda_{\mathrm{n},j} = 0$ for all $j \in \K$.
It is left to determine $\alpha_j$ for all $j \in \K$ and thus implicitly all $\theta_i$, for all $i \in \I$.
By fixing the already known variables in \eqref{eq:step_dcs} we obtain the DAE:
 \begin{subequations}\label{eq:step_dae}
 	\begin{align}
 		&\dot{x} = F_{\mathcal{I}}(x,u)\; \theta_{\mathcal{I}}, \\
 		&\theta_i - \prod_{j \in \C_i}  \frac{1-\hat{S}_{i,j}}{2}+\hat{S}_{i,j}\alpha_j = 0,\; i\in\I, \label{eq:step_dae_theta}\\
 		&c_j(x) = 0,\;  j\in \K \label{eq:step_dae_c}.
 	\end{align}
 \end{subequations}
Recall that  $\alpha_j$ for all $j \in \mathcal{C}\setminus\mathcal{K}$ are known and thus no degrees of freedom.
We keep them for ease of notation.
Thus we have a DAE with $|\I| + |\K|$ unknowns, namely $\theta_{\I}$ and $\alpha_{\K}$, and $|\I| + |\K|$ algebraic equations in \eqref{eq:step_dae_theta} and \eqref{eq:step_dae_c}.


Next, we show that the DAE \eqref{eq:step_dae} is well-posed.
For this purpose, we define the matrix
\begin{align*}
W_{\K,\I}(x) &= \nabla c_{\K}(x)^\top F_{\I}(x) \in \R^{|\K| \times |\I|}
\end{align*}
Moreover, we define a compact notation for the partial Jacobian of \eqref{eq:step_dae_theta} w.r.t. to $\alpha_{\K}$
\begin{align*}
&B_{\K,\I}(\alpha) \coloneqq \\
&\Big[\frac{\partial}{\partial \alpha_{j}} \prod_{l \in \mathcal{C}_i}  \frac{1-\hat{S}_{i,l}}{2}+\hat{S}_{i,l}\alpha_l \mid i \in \I, j \in \mathcal{K} \Big] \in \R^{|\I| \times |\mathcal{K}|}.
\end{align*}

\begin{assumption}\label{ass:solution_existence_step}
	Given a fixed active set $\I(x(t)) = \I$ for $t \in  \mathcal{T}$, it holds that the matrix $W_{\mathcal{K},\I}(x) B_{\mathcal{K},\I}(\alpha)$ has rank~$|\K|$ , i.e. it is full rank, for all $t\in \mathcal{T}$.
\end{assumption}

\begin{proposition}\label{eq:step_dae_fixed_active_set}
Suppose that Assumption \ref{ass:solution_existence_step} holds.
Given an initial value $x(0)$, the DAE \eqref{eq:step_dae} has a unique solution for all $t\in \mathcal{T}$.
\end{proposition}
\textit{Proof.}
First, we differentiate \eqref{eq:step_dae_c} w.r.t. to $t$ to obtain a DAE of index 1:
 \begin{subequations}\label{eq:step_dae_index1}
	\begin{align}
		&\dot{x} = F_{\mathcal{I}}(x,u)\; \theta_{\mathcal{I}}, \\
		&\theta_i - \prod_{j \in \C_i}  \frac{1-\hat{S}_{i,j}}{2}+\hat{S}_{i,j}\alpha_j = 0,\; i\in\I, \label{eq:step_dae_index1_theta}\\
		&W_{\K,\I}(x) \theta_\I = 0 \label{eq:step_dae_index1_c}.
	\end{align}
\end{subequations}
It is sufficient to prove that the Jacobian of \eqref{eq:step_dae_index1_theta}-\eqref{eq:step_dae_index1_c} w.r.t. to $(\theta_{\I},\alpha_{\K})$ has rank $|\I| + |\K|$.
Then, we can apply the implicit function theorem and express the algebraic variables $(\theta_{\I}(x),\alpha_{\K}(x))$ as functions of $x$.
Since all involved functions are Lipschitz continuous, it follows that $\theta_{\I}(x)$ is Lipschitz continuous for a fixed $\I$ on $t\in\mathcal{T}$.
Consequently, the DAE \eqref{eq:step_dae_index1} reduces to an ODE with a Lipschitz continuous r.h.s..
This enables us to apply the Picard-Lindelof Theorem to obtain the assertion of the proposition.

We omit the dependencies on $\alpha$ and $x$ for brevity.
The Jacobian of \eqref{eq:step_dae_index1_theta}-\eqref{eq:step_dae_index1_c} w.r.t. to $(\theta_{\I},\alpha_{\K})$
has the form
\begin{align*}
A =	\begin{bmatrix}
		I_{|\I|} & -B_{\K,\I}\\
		W_{\K,\I} & \mathbf{0}
	\end{bmatrix}.
\end{align*}
Suppose that that there is a nonzero solution $(v,w)\in \R^{|\I|} \times \R^{|\K|}$ to
\begin{align}\label{eq:linear_sys_step_dae}
	\begin{bmatrix}
		I_{|\I|} & -B_{\I,\K}\\
		W_{\K,\I} & \mathbf{0}
	\end{bmatrix}
\begin{bmatrix}
		v \\w
	\end{bmatrix} = 0.
\end{align}
From the first line we have $v = B_{\I,\K}w$ and inserting this into the second line we have
$W_{\I,\K}B_{\I,\K}w = 0$. Since matrix $W_{\I,\K}B_{\I,\K}\in \R^{|\K|\times |\K|}$ has rank $|\K|$, the only solution to \eqref{eq:linear_sys_step_dae} is $w =0$ and $v = Bw = 0$. Hence, $A$ has full rank. \qed

%The assumption on matrix $W_{\K,\I}B_{\K,\I}$ is arguably more technical and less instructive than the equivalent assumption for Stewart's formulation.
%It would be helpful to obtain the same result with more instructive assumptions on $W_{\K,\I}$ and $B_{\K,\I}$.
%We observed in practice that $B_{\K,\I}$ has always full column rank for $\alpha_{\K} \in (0,1)$.
%However, assuming $W_{\K,\I}$ to be of rank $|\K|$, together with the full rank of $B_{\K,\I}$ is not sufficient to guarantee for $W_{\K,\I}B_{\K,\I}$ to be full rank.
%This can be seen from the counter-example where $W = \begin{bmatrix}I_{|\K|} \;\mathbf{0}\end{bmatrix}$ and $B = \begin{bmatrix}
%	\textbf{0}\\
%	I_{|\K|}
%\end{bmatrix}$, $\mathrm{rank}(WB) < |\K|$.

In \cite{Dieci2011} the authors make some assumptions on the signs of the entries of $W_{\K,\I}(x)$ and prove the existence, but not uniqueness, of solutions with a fixed-point argument.
For the case of $|\mathcal{K}| \leq 2$, i.e., sliding modes with co-dimension 1 or 2, they even prove the uniqueness of solutions with appropriate assumptions on the signs of the entries of $W_{\K,\I}(x)$.


We remind the reader that for a given $x(t)$ there might be several $\I$ that yield meaningful DAEs of the form of Eq. \eqref{eq:step_dae}.
This may happen when the Filippov DI does not have unique solutions, such as in Example \ref{ex:switching_cases} case (d).

\begin{comment}
\color{red}
\begin{remark}
	It would be nice to have more instructive assumptions than Assumption \ref{ass:solution_existence_step}.
	\begin{lemma}[Corollary 6.1 in \cite{Matsaglia1974}]
	Let $A_1 \in \R^{k \times n }$ and $A_2 \in \R^{n \times q}$, then
	\begin{align*}
		\mathrm{rank}(A_1)+	\mathrm{rank}(A_2) - n \leq 	\mathrm{rank}(A_1 A_2) \leq \min(\mathrm{rank}(A_1),	\mathrm{rank}(A_2)).
	\end{align*}
	\end{lemma}
	Using this lemma and assuming both $B$ and $W$ to be full rank $|\K|$ we obtain
	\begin{align*}
		2|\K|-|\I|\leq \mathrm{rank}(WB) \leq |\K|.
	\end{align*}
	This is clearly not tight and is somewhat confirmed by my counterexample above.
	It would be nice to prove that the matrix $B$ has rank $|K|$. I observed in practice that it always
	holds for $\alpha_{\mathcal{K}} \in (0,1)$, but I failed to find an obvious proof.
	For 2D it looks like
	\begin{align}
		B(\alpha) & =\begin{bmatrix}
		\alpha_2 &\alpha_1\\
		1-\alpha_2 & -\alpha_1\\
		-\alpha_2 &\ 1-\alpha_1\\
		-(1-\alpha_2) & -(1-\alpha_1)
		\end{bmatrix}
	\end{align}
\end{remark}
\color{black}
\end{comment}
\begin{comment}
\subsection{Predicting a new active set}\label{sec:step_predicting_active_sets}
Recall that in Stewart's representation, we have
$\mathcal{I}(x) = \{ i \in \mathcal{J} \mid g_i(x) = \min_{j\in \mathcal{J}}g_j(x)\}$.
The definition of $\mathcal{I}(x)$ via the switching functions $c_j(x)$ is slightly more involved.
This can be seen from the definition:
\begin{align}\label{eq:active_set_via_theta}
	\I(x) = \{ i \in \J \mid \theta_i > 0\},
\end{align}
and the fact that $\theta_i$ is related to the functions $c_j(x)$ in a more complicated way.
Using Eq. \eqref{eq:theta_via_step} and \eqref{eq:active_set_via_theta} we obtain:
\begin{align*}
%	\label{eq:index_set_via_swiching_fun}
	\I(x) = \Big\{ i \in \J \mid \prod_{j=1}^{n_c} \frac{1+\hat{S}_{i,j}}{2}+\hat{S}_{i,j}\gamma(c_j(x))>0\Big\}.
\end{align*}
The LCP in \cite[Theorem 3.2]{Stewart1990a} is constructed from the total time derivative of $\lambda$.
Here, we would need to use the total time derivatives of $\lambdap$ and $\lambdan$.
It is clear from Eq. \eqref{eq:step_dcs} that we cannot easily obtain an LCP which relates $\dot{\lambda}_{\mathrm{p}}$, $\dot{\lambda}_{\mathrm{n}}$ and $\theta$.
Therefore, we omit to derive such an auxiliary problem for predicting the next action set at a switching point.
The price we pay is that we need slightly more restrictive assumptions to prove the convergence of the FESD scheme for the step reformulation \eqref{eq:step_dcs} in the next chapter.
However, omitting this step has no consequences for the derivation of the FESD scheme \eqref{eq:step_dcs} nor is it used in the computations.
\end{comment}
\section{Efficient representation of the regions}
union, geomertry, lifting
\subsection{Representing unions of sets}\label{sec:unions_of_sets}
Sometimes the regions $R_i$ are given as unions of sets defined via the switching functions $c(x)$.
Once again, we illustrate the idea with a simple example and discuss the general case in the sequel.
\begin{example}[Union of sets]\label{ex:union_of_sets}
We regard an example with two scalar switching functions $c_1(x)$ and $c_2(x)$ that define the two regions:
\begin{alignat*}{4}
R_1 &&\,=\, &\{ x\in \R^{n_x} \mid c_1(x)>0\} \\
    &&\cup\, &\{ x\in \R^{n_x} \mid c_1(x)\leq 0,\, c_2(x)>0 \},\\
R_2 &&\,=\, &\{ x\in \R^{n_x} \mid c_1(x)< 0,\, c_2(x)<0 \}.
\end{alignat*}
It can be seen that the related Filippov system reads as $\dot{x} = \theta_1 f_1(x) + \theta_2 f_2(x)$, where
\begin{align*}
\theta_1 & = \alpha_1 + (1-\alpha_1) \alpha_2,\;
\theta_2  =(1-\alpha_1) (1-\alpha_2).
\end{align*}
by direct calculation, we verify that $\theta_1,\theta_2 \geq 0$ and $\theta_1 + \theta_2 = 1$.
In contrast to the previous examples, the union of sets introduces a sum in the expressions for $\theta_1$.
We define the sign matrix
\begin{align*}
\hat{S}&=\begin{bmatrix}
1 &0\\
-1 &1 \\
-1 &-1
\end{bmatrix}
\end{align*}
and a the matrix summarizing the dynamics $F(x) = \begin{bmatrix} f_1(x) & f_1(x)&f_2(x) \end{bmatrix}$.
The first two entries of $F(x)$ are identical, thus the expression for $\theta_1$ is the sum of the expressions obtained for the first two rows of $\hat{S}$ via Eq. \eqref{eq:theta_via_step}.
\end{example}
We generalize the reasoning above as follows.
Given $n_f$ total regions and the  matrix $F(x,u) \in \R^{n_x} \times \R^{n_F}$, where $n_F \geq n_f$ is the number of possibly repeating columns.
We define the index sets $\I_k = \{ i \mid F_{\bullet,i}(x,u) = f_k(x,u) \}$, i.e., sets of column indices that are equal to $f_k(x,u)$.
This definition is accompanied by an appropriate sign matrix $\hat{S} \in \R^{n_F \times n_c}$.
Note that if we have no unions, then $n_F = n_f$ and $\I_k = \{k\}$ for all $k \in \I$.
Using these definitions, the expression for $\theta_i$ via step functions reads as:
\begin{align}\label{eq:theta_via_step_union}
	\theta_i &= \sum_{k \in \I_i}  \prod_{j\in \C_k}  \frac{1-\hat{S}_{k,j}}{2}+\hat{S}_{k,j}\alpha_j.
\end{align}
\subsection{Summary of expressions for $\theta$ via step functions}
We summarize the developments above and provide an overview of how are the elementary algebraic expressions for the multipliers $\theta_i$ are related to the geometric definition of the regions $R_i$.
All other more complicated expressions can be obtained by using the one listed in Table \ref{tab:step_summary}.
For this purpose let us regard the following two sets:
$R_{j} = \{x \mid c_j(x) > 0\}$ and $R_{k} = \{x \mid c_k(x) > 0 \}.$

\begin{table}[t]
	\centering
	\centering
	\begin{tabular}{p{5.3cm}p{2.0cm}}
		\hline
		\text{Definition} $R_i$ & \text{Expression} $\theta_i$\\
		\hline
		$R_i = R_j$ & $\alpha_j$ \\
		$R_i = R_{j}\cup R_k $& $\alpha_j + \alpha_k$\\
		$R_i = R_{j}\cap R_k$ & $\alpha_j  \alpha_k$\\
		$R_i = \mathrm{int}(\R^{n_x} \setminus R_{j}) = \{x \mid c_j(x)<0\}$ & $1-\alpha_j$ \\
		$R_i = R_{j} \setminus R_k$ & $\alpha_j- \alpha_k$\\
		\hline
	\end{tabular}
	\caption{Summary for expressions of $\theta_i$ depending on the definition of $R_i$.}
	\label{tab:step_summary}
\end{table}

\begin{remark}[Sum of Filippov systems]
In practice, one often encounters DIs that arise from the sum of several Filippov systems.
This occurs for example, if we have multiple surfaces with friction, or multiple objects touching the same frictional surface \cite{Stewart1996}.
All developments from this paper can be extended to this case and are implemented in NOSNOC.
For sake of brevity, we omit the corresponding equations and refer the reader to~\cite{Nurkanovic2022}.
\end{remark}

\begin{comment}
\subsection{Sum of Filippov systems via the step representation}
\label{sec:cartesian_filippov_step}
We also provide the extension of \eqref{eq:step_dcs} for the case when we have a sum product of several Filippov subsystems.
We regard $\Nsubsys$ independent subsystems where each subsystem has $n_f^k$ modes.
We equip the variables of every subsystem with a superscript, e.g., $\theta^k \in \R^{n_{f}^{k}}$ for all $k \in \{1,\ldots,\Nsubsys\}$.
All other variables are defined accordingly.
Every mode's convex combination is encoded by its parametric LP of the form \eqref{eq:step_parametric_lp} which is formulated with the subsystems' switching functions $c^k(x) \in \R^{n_c^k}$  for all $k \in \{1,\ldots,\Nsubsys\}$.
Instead of \eqref{eq:filippov_di_with_multiplers} one can write:
\begin{align}\label{eq:filippov_di_with_multiplers_multiple2}
	\dot{x} \in \Big\{ \sum_{k =1}^{\Nsubsys} \! \sum_{i= 1}^{n_f^k} \theta_{i}^k f_{i}^k (x,u) \ \mid\ &\sum_{i= 1}^{n_f^k} \theta_{i}^k =1,\\ \nonumber &
\theta^k \geq 0, \; k = 1,\dots, \Nsubsys \Big\}.
\end{align}
Thus, following a similar reasoning as in Section \ref{sec:step_dcs} one can derive the DCS:
\begin{subequations}\label{eq:step_dcs_multiple_step}
	\begin{align}
		\dot{x}  & = \sum_{k=1}^{\Nsubsys} F^k(x,u ){\theta}^k ,\\
    	&{\theta}_i^k = \prod_{j\in \C_i^k}  \frac{1-\hat{S}^k_{i,j}}{2}+\hat{S}^k_{i,j}\alpha_j^k,\;
    	&\textrm{for all } i\in \J^k\\
		&{c}^{k}(x) = {\lambda}^{\mathrm{p},k} - {\lambda}^{\mathrm{n},k},\\
		&0 \leq  {\lambda}^{\mathrm{n},k} \perp {\alpha}^{k} \geq 0,\\
		&0 \leq  {\lambda}^{\mathrm{p},k} \perp e-{\alpha}^{k}\geq 0,\\
		&& \textrm{for all } k\in \{1,\ldots,\Nsubsys\} \nonumber
	\end{align}
\end{subequations}
where $F^k(x,u) = [f_{1}^{k}(x,u),\ldots,f_{n_f^k}(x,u)^{k}] \in \R^{n_x \times n_f^k}$ collects all vector fields of the subsystem $k$.
Similarly, ${\lambda}^{\mathrm{p},k}, {\lambda}^{\mathrm{n},k}, {\alpha}^{k}  \in \R^{n_c^k}$ are the remaining algebraic variables of the $k-$th subsystem.
For ease of notation, in the remainder of this paper, we treat the case with $\Nsubsys = 1$.
\end{comment}
\subsection{A lifting algorithm for the multi-affine terms}\label{sec:step_lifting_algortihm}
Depending on how many nonzero entries $\hat{S}_{i,\bullet}$ has, the expression for $\theta_i$ in Eq. \eqref{eq:theta_via_step} might be very nonlinear since it is a product of $|\C_i|$ affine terms.
To reduce the nonlinearity, we introduce auxiliary lifting variables as in the \textit{lifted} Newton's method \cite{Albersmeyer2010}, which iterates on a larger but less nonlinear problem.
Here, we apply this approach to the expressions in Eq. \eqref{eq:theta_via_step} involving multi-affine terms with $\alpha_j$.
%Denote by $n_{R_i} = |\C_i|$ the number of non-zero entries in $\hat{S}_{i,\bullet}$.
%This is also the number of scalar switching functions involved in the definition of the regions $R_i$.
Whenever we have more than two terms in the multi-affine expression for $\theta_i$, we introduce lifting variables $\beta_k$ to end up with an equivalent formulation that has only bilinear terms.
We exploit the structure of the matrix $\hat{S}$ and derive an easy-to-implement algorithm that automates the lifting procedure.
% in the expressions for $\theta_i$.


To give an idea of the final results we aim to obtain, we illustrate the lifting procedure w a simple example.
\begin{example}\label{ex:step_lifting}
Regard a PSS with $n_c=4$ switching functions and $n_f = 4$ modes, where the matrix $\hat{S}\in \R^{4\times4}$ reads as:
	\begin{align*}
		\hat{S} = \begin{bmatrix}
			1 & 0 &0 &0\\
		    -1& 1& 0 & 0\\
			-1& -1& -1 & 1\\
			-1& -1& -1 & -1\\
		\end{bmatrix}
	\end{align*}
Using Eq. \eqref{eq:theta_via_step} we have:
\begin{align*}
G_{\mathrm{step}}(\theta,\alpha) &=
\begin{bmatrix}
\theta_1 \shortminus \alpha_1\\
\theta_2 \shortminus (1\shortminus\alpha_1)\alpha_2\\
\theta_3 \shortminus (1\shortminus\alpha_1)(1\shortminus\alpha_2)(1\shortminus\alpha_3)\alpha_4\\
\theta_4 \shortminus (1\shortminus\alpha_1)(1\shortminus\alpha_2)(1\shortminus\alpha_3)(1\shortminus\alpha_4)
\end{bmatrix} = 0.
\end{align*}
ithThe last two terms are quite nonlinear.
 We can introduce the lifting variable
$\beta \in \R^2$ and obtain
\begin{align*}
&G_{\beta}(\alpha,\beta) =
	\begin{bmatrix}
			\beta_1 - (1-\alpha_1)(1-\alpha_2)\\
		\beta_2 - \beta_1(1-\alpha_3)
	\end{bmatrix}=0,\\\
&G_{\theta}(\theta,\alpha,\beta)
=\begin{bmatrix}
 	\theta_1 - \alpha_1\\
 	\theta_2 - (1-\alpha_1)\alpha_2\\
 	\theta_3 - \beta_2\alpha_4\\
 	\theta_4 - \beta_3(1-\alpha_4)
 	\end{bmatrix}=0
\end{align*}
The equation $G_{\beta}(\alpha,\beta)=0$ relates the lifting variables $\beta_i$ with the $\alpha_j$, whereas $G_{\theta}(\theta,\alpha,\beta)$ provides new expressions for $\theta_i$ via $\beta_i$ and the remaining $\alpha_j$.
By replacing $G_{\mathrm{step}}(\theta,\alpha)= 0$ with $G_{\mathrm{lift}}(\theta, \alpha,\beta)  \coloneqq
(G_{\beta}(\alpha,\beta),	G_{\theta}(\theta,\alpha,\beta) ) =0$, we obtain an equivalent system of equations that only consists of bilinear terms.
\end{example}


\begin{algorithm}\label{algo:lifting}
	\caption{Lifting algorithm for the step DCS \eqref{eq:step_dcs}}
	\label{alg:lifting_dcs}
	\begin{algorithmic}[1]
		\State \textbf{Input:} $\hat{S}, n_{\mathrm{depth}}$
		\State \textbf{Initialize:}
%		Either $\hat{S}^{\mathrm{temp}}$ or $\tilde{S}$
%		Either $\\theta^{\mathrm{temp}}$ or $\tilde{\theta}$
%		Either $N^{\mathrm{temp}}$ or $\tilde{N}$
		$\tilde{S} \leftarrow \hat{S}$,
		$k  \leftarrow 0$;
%		$\ILift \leftarrow \emptyset$,
		$\tilde{\theta} \leftarrow e \in \R^{n_f}$,
		$G_{\theta}(\theta,\alpha,\beta) \leftarrow [\;]$,
		$G_{\beta}(\alpha,\beta) \leftarrow [\;]$.
		\For{$j=1:n_c$}
		\State $\tilde{N} \leftarrow \sum_{j=1}^{n_c} |\tilde{S}_{\bullet,j}|$
		\State $\ILift \leftarrow \{ i \mid \tilde{N}_i = j \}$
		\State
		$\tilde{\theta} \leftarrow
		\tilde{\theta} \cdot  \Big(\frac{e-\tilde{S}_{\bullet,j}}{2}+\hat{S}_{\bullet,j}^{\mathrm{temp}}\cdot \alpha_j \Big)$
		% add theta expression
		\If {$\ILift \neq \emptyset $}
		\State
		$ G_{\theta}(\theta,\alpha,\beta) \leftarrow
		(G_{\theta}(\theta,\alpha,\beta),
		\theta_{k+\ILift}- \tilde{\theta}_{\ILift})$
		\State
		Remove entries of $\tilde{\theta}$ with index in $\ILift$
		%		$\tilde{\theta}  \leftarrow [\tilde{\theta}_i \mid i \notin\ILift]$
		\State
		Remove rows of $\tilde{S}$ with index in $\ILift$
		%		$\tilde{S} \leftarrow [ \tilde{S}_{i,j} \mid i\notin \ILift, j \in \mathcal{C}]$
		\State
		$k \leftarrow k+\max(\ILift)$
		\EndIf
		\If{ $j \in \{ n_{\mathrm{depth}},\ldots,n_c-1\}$}
		\State
		$\{ \I_{\mathrm{red}},\I_{\mathrm{full}}\} =
		\texttt{unique}(\tilde{S}_{\bullet,\{1,\ldots,j\}})$,
		\State $\beta \leftarrow (\beta,\beta^{j})$ where  $\beta^j \in \R^{|\I_{\mathrm{red}}|}$
		\State $G_{\beta}(\alpha,\beta) \leftarrow
		(G_{\beta}(\alpha,\beta)
		\beta^j - \tilde{\theta}_{\I_{\mathrm{red}}})$
		\State $\tilde{\theta} \leftarrow \beta^j_{\I_{\mathrm{full}}}$
		\EndIf
		\EndFor
		\State  $G_{\mathrm{Lift}}(\theta,\alpha,\beta) \coloneqq (G_{\theta}(\theta,\alpha,\beta),G_{\beta}(\alpha,\beta))$
		\State \textbf{Output:} $G_{\mathrm{Lift}}(\theta,\alpha,\beta)$ , $\beta$
	\end{algorithmic}
\end{algorithm}

We proceed with outlining a general lifting algorithm.
The expressions for $\theta_i$ consist of the product of $|\C_i|$ affine terms.
Our goal is to have at most $n_{\mathrm{depth}}$ terms in the multi-affine expression for $\theta_i$.
With the parameter $n_c \geq n_{\mathrm{depth}} \geq 2$, we control the number of terms in the multi-affine expressions and implicitly the number of new lifting variables $\beta \in \R^{n_\beta}$.
Without loss of generality, we assume that the number of nonzero entries in the rows of the matrix $\hat{S}$  is monotonically increasing.
Given the matrix $\hat{S}$, our goal is to automatically obtain the constraint $G_{\mathrm{lift}}(\theta,\alpha,\beta)=0$.

The algorithm outlined above can be implemented using a symbolic framework such as \texttt{CasADi} \cite{Andersson2019}.
We provide the pseudo code in Algorithm \ref{alg:lifting_dcs}, which introduces the lifting algebraic variables $\beta$ and new \textit{lifted} expressions for $\theta_i$, namely $G_{\mathrm{lift}}(\theta,\alpha,\beta)$.
We briefly comment on some of the most important steps in this algorithm.
Note that we make use of three helper variables, the matrix $\tilde{S}$ and the vectors $\tilde{\theta}$ and $\tilde{N}$.
The matrix $\tilde{S}$ is a submatrix of $\hat{S}$, where we have removed the rows with index $i$, for which we already have a (lifted) expression for $\theta_i$.
The vector $\tilde{N}$, defined in line 4, collects the number of nonzero entries of every row $\tilde{S}$.
In other words, it keeps track of how many terms are in the initial expressions for $\theta_i$, that is not yet lifted.

The main for loop iterates from $j = 1$ to $n_c$ and provides in every iteration the expressions for all $\theta_i$ that have exactly $j$ terms in their multi-affine expression.
The index set  $\ILift = \{ i \mid \tilde{N}_i = j \}$, defined in line 5, contains the indices of $\theta$, that have exactly $j$ entries in their corresponding multi-affine expression.
In line 6 we define the auxiliary variable $\tilde{\theta}$ which stores the intermediate expressions for $\theta$ with up to $j$ terms in the product.
The index $k$ stores the index of the last $\theta_k$ for which a lifted expression was derived.
For $j \leq n_{\mathrm{depth}}$ the expressions for $\theta_i$ are unaltered.
This is treated in lines 7-11.


On the other hand, for $j > n_{\mathrm{depth}}$ we introduce new lifting variables
$\beta^j$ (line 15) and change the expression for $\tilde{\theta}$ accordingly.
This is done in lines 13-17.
A key tool is the function \texttt{unique} in line 14.
It is available in \texttt{MATLAB} and in the \texttt{numpy} package in \texttt{python}.
It works as follows, given a matrix $A \in \R^{m \times n}$ it returns the matrix $\tilde{A} \in \R^{p \times n}$, with $p \leq m$.
This is the matrix constructed from $A$ by removing its repeating rows.
More importantly for our needs, it returns the index sets $\I_{\mathrm{red}}$ and $\I_{\mathrm{full}}$, with the properties
$A =  \begin{bmatrix}
		\tilde{A}_{i,\bullet} \mid i \in \I_{\mathrm{full}}
	\end{bmatrix}$
and
$\tilde{A} =  \begin{bmatrix}
	{A}_{i,\bullet} \mid i \in \I_{\mathrm{red}}
\end{bmatrix}$.
Note that $|\I_{\mathrm{red}}| = p$  and $|\I_{\mathrm{full}}| = m$.
This enables the use of the same $\beta^j$ for several $\theta_i$ if they share the same terms in the according multi-affine expressions, cf. lines 15-17.
After the loop is finished, the algorithm outputs $G_{\mathrm{Lift}}(\theta,\alpha,\beta)$ and $\beta$.
One can verify that Algorithm \ref{alg:lifting_dcs} produces the same output as Example~\ref{ex:step_lifting}.



\begin{comment}
\begin{example}
	Example of algorithm output for
	\begin{align*}
		S &= \begin{bmatrix}
			1  & 0 & 0 & 0 & 0 \\
			-1  & 1 & 0 & 0 & 0 \\
			-1  & -1 & 1 & 0 & 0 \\
			-1  & -1 & -1 & 1 & 0 \\
			-1  & -1 & -1 & -1 & 1 \\
			-1  & -1 & -1 & -1 & -1 \\
		\end{bmatrix} \in \R^{6 \times 5}
	\end{align*}
	the vector $\theta$ after lifting and the intermediate lifting variables are defined as
	\begin{align*}
		g_{\mathrm{lift},\theta}(\theta,\alpha,\beta) &= \theta - \begin{bmatrix}
			\alpha_1\\
			(1-\alpha_1)\alpha_2\\
			\beta_{1,1} \alpha_3\\
			\beta_{2,1} -\alpha_4\\
			\beta_{3,1} \alpha_5\\
			\beta_{3,1} (1-\alpha_5)
		\end{bmatrix}, \;
		g_{\mathrm{lift},\beta}(\alpha,\beta)  = \begin{bmatrix}
			\beta_{1,1} - (1-\alpha_1)(1-\alpha_2)\\
			\beta_{2,1} - \beta_{1,1}(1-\alpha_3)\\
			\beta_{3,1} - 	\beta_{2,1}(1-\alpha_4)
		\end{bmatrix}.
	\end{align*}
	All algebraic variables are $(\theta,\beta,\alpha,\lambda_1,\lambda_0)$.
	In Stewart's representation, this would require $32+32+1 = 65$ algebraic variables, and this representation needs only $6+3+3\cdot5 = 24$ algebraic variables.
\end{example}
\end{comment}

\begin{comment}
\color{blue}
Alternative (more compact) definition?
Let $\mathcal{K}_i = \{ k \mid \hat{S}_{i,k}\neq 0\}$,
then
\begin{align*}
	F_{\mathrm{S}}(x) &\coloneqq \Big\{ \sum_{i=1}^{\Nsys} \prod_{j \in \mathcal{K}_i}\Big( \frac{1-\hat{S}_{i,j}}{2}+\hat{S}_{i,j}\alpha_i \Big) f_i(x) \mid \alpha \in \Gamma(c(x)) \Big\}.
\end{align*}
\begin{align*}
	\theta_i = \prod_{j \in \mathcal{K}_i} \frac{1-S_{i,j}}{2}+S_{i,j}\alpha_j,\\
\end{align*}

\begin{align}
	\theta_i = 2^{n_{c}-n_{R_i}}  \det(\mathrm{diag}((\frac{1}{2}(e-S_{i,\bullet})+\mathrm{diag}(S_{i,\bullet})\alpha))
\end{align}

\begin{align}
	\I(x) = \Big\{ i \in \mathcal{J} \mid \prod_{j=1}^{n_c}  \frac{1+\hat{S}_{i,j} \sign(c_j(x))}{2}>0\Big\}.
\end{align}
alternative:
\color{black}
\end{comment}


\begin{comment}
	\begin{algorithm}\label{algo:lift}
		\caption{Lifting algorithm for the Step DCS \eqref{eq:step_dcs}}
		\label{alg:lift_ap_dcs}
		\begin{algorithmic}[1]
			\State \textbf{Input:} $\{ \hat{S}, \theta, \alpha, n_{\mathrm{depth}}\}$
			\State \textbf{Initialize:} $\tilde{S} \leftarrow \hat{S}$, $\tilde{G}(\cdot) \leftarrow e \in \R^{n_f}$,$i_\texttt{prog}  \leftarrow 0$; $\I \leftarrow \emptyset$, $\I_\texttt{done} \leftarrow \emptyset$, $n_{\mathrm{lift}} \leftarrow n_f$,$n_{\beta} \leftarrow 0$;
			\Procedure{Lifting}{$\theta,\alpha,\beta$}
			\For{$i=1:n_c$}
			\State $n_{R} = \sum_j^{n_c} |\tilde{S}_{\bullet,j}|$
			\Statex \textcolor{gray}{\% Define index sets of ...\%}
			\State $\I \leftarrow \texttt{find}(n_{R} \geq i)$
			\State $\I_{\texttt{done}} \leftarrow \texttt{find}(n_{R} = i)$
			\Statex \textcolor{gray}{\%Update vector of temporal lifting variables.\%}
			\State
			$
			\tilde{g}(\cdot) \leftarrow \mathrm{diag}(\tilde{g}(\cdot)) \cdot  \Big(\frac{e-\tilde{S}_{\texttt{ind},i}}{2}+\tilde{S}_{\I,i}\cdot ( \alpha_i \; e)\Big)
			$
			\Statex \textcolor{gray}{\% Define expression for $\theta$ via bilinear terms. \%}
			\If{$\texttt{is\_not\_empty}(\I_{\mathrm{done}})$}
			\State
			$
			g_{\mathrm{lift,\theta}}(\cdot) \leftarrow (g_{\mathrm{lift,\theta}},\theta_{\I+i_\texttt{prog}} - \tilde{g}_\texttt{ind\_done}(\cdot))
			$
			\State
			$
			\tilde{g}_{\I_\texttt{done}} \leftarrow [\;],\;
			\tilde{S}_{\I_\texttt{done},\bullet} \leftarrow [\;],\;
			i_\texttt{prog}\leftarrow i_\texttt{prog} +\mathrm{max}(\I_\texttt{done})
			$
			%		 \State		 \begin{align*}
				%			 \tilde{g}_{\I_\texttt{done}} &\leftarrow [\;],\
				%		 	\tilde{S}_{\I_\texttt{done},\bullet} \leftarrow [\;],\\
				%		 	i_\texttt{prog} &\leftarrow i_\texttt{prog} +\mathrm{max}(\I_\texttt{done})
				%		 \end{align*}
			\EndIf
			\Statex \textcolor{gray}{\%Define lifting variables $\beta$ for current layer.\%}
			\If{ $i \in \left[ n_{\mathrm{depth}},n_c \right) $}
			\Statex
			{\textcolor{gray}{ \% Return the matrix $\hat{S}$ which consists of the non-repeating rows of $\tilde{S}$ and two index vectors $\I_{\tilde{S}{\mathrm{a}}},\I_{\tilde{S}{\mathrm{b}}}$ such that ... \%}}
			\State $\{ \hat{S},\I_{\tilde{S}{\mathrm{a}}},\I_{\tilde{S}{\mathrm{b}}}\} = \texttt{unique\_rows}(\tilde{S}(:,i))$, $n_\beta \leftarrow n_\beta+n_{\beta,i}$;
			\State $n_{\beta,i} \leftarrow \texttt{number\_of\_rows}(\hat{S})$, $n_{\mathrm{lift}} \leftarrow n_{\mathrm{lift}}+n_{\beta,i}$;
			\State $\beta_i \leftarrow (\beta_{i,j} \mid j\in \{1,\ldots,n_{\beta,i}\})\in \R^{n_{\beta,i}}$;
			\State $\beta \leftarrow (\beta,\beta_{i})$
			\State $g_{\mathrm{lift},\beta}(\cdot) \leftarrow (g_{\mathrm{lift},\beta}(\cdot)- \tilde{g}_{\I_{\tilde{S},\mathrm{a}}}(\cdot))$;
			\Statex \textcolor{gray}{\%Update vector of temporal lifting variables.\%}
			\State $\tilde{g}(\cdot) \leftarrow \beta_{i,\I_{\tilde{S}{\mathrm{b}}}}$;
			\EndIf
			\EndFor
			\State  $g_{\mathrm{lift}}(\cdot) \leftarrow (g_{\mathrm{lift},\theta}(\cdot) ,g_{\mathrm{lift},\beta}(\cdot)) \in \R^{n_{\mathrm{lift}}}$
			\EndProcedure
			\State \textbf{Output:} $\{g_{\mathrm{lift}}(\cdot),\beta,n_{\mathrm{lift}},n_{\beta}\}$
		\end{algorithmic}
	\end{algorithm}
\end{comment}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../fesd_step_article"
%%% End:

